EDAF: An End-to-End Delay Analytics Framework for 5G-and-Beyond Networks

Supporting applications in emerging domains like cyber-physical systems and human-in-the-loop scenarios typically requires adherence to strict end-to-end delay guarantees. Contributions of many tandem processes unfolding layer by layer within the wireless network result in violations of delay constraints, thereby severely degrading application performance. Meeting the application's stringent requirements necessitates coordinated optimization of the end-to-end delay by fine-tuning all contributing processes. To achieve this task, we designed and implemented EDAF, a framework to decompose packets' end-to-end delays and determine each component's significance for 5G network. We showcase EDAF on OpenAirInterface 5G uplink, modified to report timestamps across the data plane. By applying the obtained insights, we optimized end-to-end uplink delay by eliminating segmentation and frame-alignment delays, decreasing average delay from 12ms to 4ms.

==> backups/0_introduction_bckup.tex <==
\section{Introduction}

%Why predict wireless communication behaviour?
The increasing demand of latency-critical applications in Cyber-Physical Systems (CPS) and Human-In-The-Loop (HITL) applications emphasizes the crucial demand for dependable wireless communication.
A dependable communication system can provably ascertain that it will deliver the required service performance for the communication services that are agreed.
For instance, the end-to-end latency of the communication must be assured not to exceed a specified target with a certain probability, and similar assurances are required for throughput-dependent services.

To address these stringent requirements, one prevailing focus in current wireless network research centers on forecasting latency or throughput using specific data-driven predictors and optimize the network to fulfill the service requirements.
To the best of our knowledge, in these works, the accuracy of the proposed predictors are investigated and optimized, however, such analysis does not provide a comprehensive understanding of how accurately a wireless link can be forecasted.
Moreover, the inherent uncertainty in wireless links poses a challenge, rendering it impossible for any algorithm to forecast link latency or throughput with absolute precision.
The concept of predictability, defined as a metric measuring the predictability of a time series of latency or throughput measurements, sets an upper bound on prediction accuracy.
Importantly, predictability is viewed as an intrinsic feature of data, independent of the predictive model employed. 

%One prevailing focus in current wireless network research centers on characterizing key performance indicators (KPIs), such as latency or throughput, using specific data-driven or model-based predictors.
%Additionally, efforts are directed towards exploring optimization strategies to enhance prediction accuracy and efficiency. 
%Despite these efforts, the inherent uncertainty in wireless links poses a challenge, rendering it impossible for any algorithm, regardless of optimization, to forecast link latency or throughput with absolute precision.
%However, the accuracy of existing predictions does not provide a comprehensive understanding of how accurately a wireless link can be forecasted.
%The concept of predictability, defined as a metric measuring the predictability of a time series of KPI measurements, sets an upper bound on prediction accuracy.
%Importantly, predictability is viewed as an intrinsic feature of data, independent of the predictive model employed. 
%For instance, even with a highly proficient predictive algorithm, the theoretical accuracy remains constrained, such as being capped at $85\%$, while the predictability stands at $85\%$.

%Forecasting plays a vital role in diverse fields, whether it's predicting future demand for long-term capital investments, scheduling call center staff for the upcoming week, or managing inventory stock requirements.
%Regardless of the timeframe or specific context, accurate forecasting is essential for effective and efficient planning to achieve certain goals.

Forecasting varies in complexity depending on the metric and its influencing factors.
Quantitative forecasting for a system metric is easily applicable when three key conditions are met: a clear understanding of contributing factors, ample numerical information from the past, and a reasonable assumption that past patterns will persist into the future.
For instance, accurate predictions of electricity demand are achievable as we comprehend the influential factors, have abundant historical data, and can develop a robust model linking demand to key variables like weather temperature.
In contrast, forecasting currency exchange rates presents challenges as only one condition is met: there is abundant data. 
Understanding the factors influencing exchange rates is limited, and the forecasts themselves impact the rates directly.
Forecasting complexity arises from the inherent concept of \emph{predictability} associated with the metric. 
Understanding the predictability of a metric is crucial in forecasting, regardless of the chosen model, as it provides insights into the inherent limits of prediction.

\subsection{Causes of Latency in Wireless Communication}



\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/latencymodel_time.pdf}
    \caption{Latency components}\label{fig:latencymodel_time}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.65\linewidth]{figures/latencymodel_queue.pdf}
    \caption{Influential factors on queuing latency}\label{fig:latencymodel_queue}
\end{figure}

As mentioned above, forecasting the key performance metrics of a system, requires a clear understanding of the influential factors in the form of a model that describes with which mechanism they contribute.
In this section, we decompose latency of a packet traveling through the wireless link as a sum of its major components and describe the causes for each.

As shown in Figure \ref{fig:latencymodel_time}, we separate the latency into wireless link latency and queuing latency.
Due to the shared and stochastic capacity of the wireless channel, application packets i.e. PDUs can be buffered upon arrival since the wireless link is busy transmitting the previous PDUs.
Also, PDUs are queued when the link i.e. server is on vacation due to not finding transmission opportunity.
In different wireless networks such buffering could occur at multiple layers, however, without loss of generality, we consider only one and we call it PDU queue.

We consider queuing delay from when the packet enters the queue until it is being consumed by MAC layer for transmission, i.e. service time.
Figure \ref{fig:latencymodel_queue} depicts the process in which the service time of a PDU, i.e. when its service starts, is determined.
First, the packet arrives and needs to wait until the previous packet in the queue departs.
Then, when no packets are in front, the service time starts at the first transmission opportunity i.e. when the link is back from vacation.

In TDD cellular networks, vacation intervals are mainly due to the division of time slots to uplink or downlink in a repeating predefined pattern.
Moreover, even when the desired uplink or downlink time slot has arrived, the link may not find it free since they could be allocated to other UEs.
In contention-based wireless networks such as WiFi, the link is capable of carrier sensing and starts transmitting when the channel is free.
The link's vacation time in such networks is less predictable.

Given the precise values of these three factors, the service time and queuing delay of the packet can be precisely determined:
\begin{enumerate}
    \item Packet arrival time,
    \item Wireless link vacation times,
    \item Previous packets' link delays. 
\end{enumerate}
Certainly the third factor makes the analysis cumbersome and requires resorting to queuing theory models for a better understanding.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/latencymodel_link.pdf}
    \caption{Influential factors on wireless link latency}\label{fig:latencymodel_link}
\end{figure}

Next, we introduce wireless link latency which focuses on the period that starts after queuing, when an appropriate transmission time is recognized for the packet and MAC layer starts the transmission.
Another model describing how major factors interact and form the link latency is demonstrated in Figure \ref{fig:latencymodel_link}. 
We describe the three major link latency components as follows:

%\subsubsection{Arrival Process}
%The service delivers the information in the form of IP packets.
%These packets' size and arrival pattern at the wireless link's interface can influence latency.
%For instance, bufferbloat effect can be caused by packet arrival bursts and add to the latency.
%Moreover, arrival process can contribute to Residual Service Time (RST).
%RST is defined as the duration from the moment the packet arrives at the link's interface to the point at which a potential transmission time slot is identified.
%In Time Division Duplex (TDD) wireless systems such as TDD 5G and WiFi7, the TDD frames are divided into uplink and downlink slots in repetitive periods.
%Therefore, the potential transmission time slot could be out of reach at the arrival of the packet.

\subsubsection{Segmentation Delay}
At the service time of the packet, the scheduler finds the available number of Physical Resource Blocks (PRBs) on that time slot.
Using that and the MCS index, the number of bytes that can be consumed from the queue is then calculated.
This is also known as Transport Block Size (TBS) in cellular systems which is usually in bytes and can be smaller than the packet size.
In such occasion, the packet gets segmented and the segments will be send on the upcoming transmission slots consecutively.
We define segmentation delay as the time difference between the transmission of the first and the last segments.
The scheduler chooses the MCS index is chosen based on the channel quality, where its goal usually is to keep the Block Error Rate (BLER) low and at the same time achieve the highest spectral efficiency.

\subsubsection{Retransmissions Delay}
Hybrid Automatic Repeat Request (HARQ) is used in most wireless communication schemes to ensure reliability by retransmitting lost or corrupted packets. 
It works by combining Forward Error Correction (FEC) with Automatic Repeat Request (ARQ) protocols, allowing for error correction.
However, it introduces additional retransmission delay for some packets.
This component of delay which is related to MCS index and channel conditions is retransmissions delay.
It is defined as the time difference between the first to the last transmission attempt of the last segment of the packet.

\subsubsection{Transmission Delay}
The delay of a single end-to-end transmission attempt by HARQ process is denoted by transmission delay. 
In other words, it is the time it takes for HARQ process to encode, modulate, and send a segment of the packet and receive, demodulate, and decode it at the receiver, regardless of the decoding result.
It also includes physical layer and propagation delay, which we assume are constant no matter which HARQ round is taking place.
We do not specify any influential factor for this component of latency mainly because it remains almost constant in different conditions.

%To further develop the understanding of wireless network's latency, one needs to emphasize on stochastic or less predictable factors.
%In this work we consider PDU size constant, also arrival process deterministic i.e. periodic with rate $f_s$.
According to the described model, by having the following factors at hand, the wireless link delay can be precisely calculated:
\begin{enumerate}
    \item Packet size,
    \item Packet service time,
    \item Tx slots and their available PRBs,
    \item MCS index,
    \item Number of retransmissions,
    \item Transmission delay.
\end{enumerate}


\subsection{Predictability Framework}



==> backups/1_system_model_bckup.tex <==
\section{End-to-End Delay Model}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/latencymodel_time.pdf}
    \caption{Latency components}\label{fig:latencymodel_time}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.65\linewidth]{figures/latencymodel_queue.pdf}
    \caption{Influential factors on queuing latency}\label{fig:latencymodel_queue}
\end{figure}

As mentioned above, forecasting the key performance metrics of a system, requires a clear understanding of the influential factors in the form of a model that describes with which mechanism they contribute.
In this section, we decompose latency of a packet traveling through the wireless link as a sum of its major components and describe the causes for each.

As shown in Figure \ref{fig:latencymodel_time}, we separate the latency into wireless link latency and queuing latency.
Due to the shared and stochastic capacity of the wireless channel, application packets i.e. PDUs can be buffered upon arrival since the wireless link is busy transmitting the previous PDUs.
Also, PDUs are queued when the link i.e. server is on vacation due to not finding transmission opportunity.
In different wireless networks such buffering could occur at multiple layers, however, without loss of generality, we consider only one and we call it PDU queue.

We consider queuing delay from when the packet enters the queue until it is being consumed by MAC layer for transmission, i.e. service time.
Figure \ref{fig:latencymodel_queue} depicts the process in which the service time of a PDU, i.e. when its service starts, is determined.
First, the packet arrives and needs to wait until the previous packet in the queue departs.
Then, when no packets are in front, the service time starts at the first transmission opportunity i.e. when the link is back from vacation.

In TDD cellular networks, vacation intervals are mainly due to the division of time slots to uplink or downlink in a repeating predefined pattern.
Moreover, even when the desired uplink or downlink time slot has arrived, the link may not find it free since they could be allocated to other UEs.
In contention-based wireless networks such as WiFi, the link is capable of carrier sensing and starts transmitting when the channel is free.
The link's vacation time in such networks is less predictable.

Given the precise values of these three factors, the service time and queuing delay of the packet can be precisely determined:
\begin{enumerate}
    \item Packet arrival time,
    \item Wireless link vacation times,
    \item Previous packets' link delays. 
\end{enumerate}
Certainly the third factor makes the analysis cumbersome and requires resorting to queuing theory models for a better understanding.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/latencymodel_link.pdf}
    \caption{Influential factors on wireless link latency}\label{fig:latencymodel_link}
\end{figure}

Next, we introduce wireless link latency which focuses on the period that starts after queuing, when an appropriate transmission time is recognized for the packet and MAC layer starts the transmission.
Another model describing how major factors interact and form the link latency is demonstrated in Figure \ref{fig:latencymodel_link}. 
We describe the three major link latency components as follows:

%\subsubsection{Arrival Process}
%The service delivers the information in the form of IP packets.
%These packets' size and arrival pattern at the wireless link's interface can influence latency.
%For instance, bufferbloat effect can be caused by packet arrival bursts and add to the latency.
%Moreover, arrival process can contribute to Residual Service Time (RST).
%RST is defined as the duration from the moment the packet arrives at the link's interface to the point at which a potential transmission time slot is identified.
%In Time Division Duplex (TDD) wireless systems such as TDD 5G and WiFi7, the TDD frames are divided into uplink and downlink slots in repetitive periods.
%Therefore, the potential transmission time slot could be out of reach at the arrival of the packet.

\subsubsection{Segmentation Delay}
At the service time of the packet, the scheduler finds the available number of Physical Resource Blocks (PRBs) on that time slot.
Using that and the MCS index, the number of bytes that can be consumed from the queue is then calculated.
This is also known as Transport Block Size (TBS) in cellular systems which is usually in bytes and can be smaller than the packet size.
In such occasion, the packet gets segmented and the segments will be send on the upcoming transmission slots consecutively.
We define segmentation delay as the time difference between the transmission of the first and the last segments.
The scheduler chooses the MCS index is chosen based on the channel quality, where its goal usually is to keep the Block Error Rate (BLER) low and at the same time achieve the highest spectral efficiency.

\subsubsection{Retransmissions Delay}
Hybrid Automatic Repeat Request (HARQ) is used in most wireless communication schemes to ensure reliability by retransmitting lost or corrupted packets. 
It works by combining Forward Error Correction (FEC) with Automatic Repeat Request (ARQ) protocols, allowing for error correction.
However, it introduces additional retransmission delay for some packets.
This component of delay which is related to MCS index and channel conditions is retransmissions delay.
It is defined as the time difference between the first to the last transmission attempt of the last segment of the packet.

\subsubsection{Transmission Delay}
The delay of a single end-to-end transmission attempt by HARQ process is denoted by transmission delay. 
In other words, it is the time it takes for HARQ process to encode, modulate, and send a segment of the packet and receive, demodulate, and decode it at the receiver, regardless of the decoding result.
It also includes physical layer and propagation delay, which we assume are constant no matter which HARQ round is taking place.
We do not specify any influential factor for this component of latency mainly because it remains almost constant in different conditions.

%To further develop the understanding of wireless network's latency, one needs to emphasize on stochastic or less predictable factors.
%In this work we consider PDU size constant, also arrival process deterministic i.e. periodic with rate $f_s$.
According to the described model, by having the following factors at hand, the wireless link delay can be precisely calculated:
\begin{enumerate}
    \item Packet size,
    \item Packet service time,
    \item Tx slots and their available PRBs,
    \item MCS index,
    \item Number of retransmissions,
    \item Transmission delay.
\end{enumerate}


==> backups/2_measurements.tex <==
%\subsection{Measurement}

%In TDD-configured wireless networks, data transmission and reception are usually separated in time slots during certain periods.
%Due to this cyclical scheduling, when a source emits small, periodic data packets, some of them may not be send instantly and need to wait until the transmission slot arrives.
%The duration from the moment the packet arrives at MAC layer to the point at which a suitable transmission time slot is identified, is called Residual Service Time (RST).


%For example in 5G, the length of a Radio Frame is always 10 ms and the length of a subframe is always 1 ms.
%Then depending on the numerology, there could exist one or multiple number of slots within a subframe.
%Each slot always contains 14 symbols but the symbol duration is varying according to the numerology.
%Slot Format indicates how each of symbols within a single slot is used. 
%It defines which symbols are used for uplink and which symbols are used for downlink within a specific slot. 
%In LTE TDD, if a subframe (equivalent to a Slot in NR) is configured for DL or UL, all of the symbols within the subframe should be used as DL or UL. 
%But in NR, the symbols within a slot can be configured in various ways as follows.
%We don't need to use every symbols within a slot (this can be a similar concept in LAA subframe where only a part of subframes can be used for data transmission).
%Single slot can be devided into multiple segments of consecutive symbols that can be used for DL , UL or Flexible.
%Theoretically we can think of almost infinite number of possible combinations of DL symbol, UL symbol, Flexible Symbol within a slot, but 3GPP allows only 61 predefined symbol combination within a slot as in following table.
%There are many different types of slot formats.
%It is to make NR scheduling flexible especially for TDD operation. By applying a slot format or combining different slot formats in sequence, we can implement various different types of scheduling as in the following example

==> backups/refs.tex <==
%https://kuiper2000.github.io/chaos_and_predictability/week1/week1.html

%https://otexts.com/fpp2/index.html
